Improved Gradient Descent Lower Bounds Beyond Nesterov

We study how far gradient descent (GD) can be accelerated by predetermined stepsizes in smooth convex optimization. Going beyond the classical $\Omega(n^{-2})$ first-order oracle lower bound of Nemirovsky and Yudin (1983), we prove an $\Omega(n^{-1.6342})$ non-anytime lower bound and an $\Omega(n^{-1.2408})$ anytime lower bound. These improve the recent $\Omega(n^{-1.932})$ non-anytime lower bound of Ma and Chen (2026) and the $\Omega(n^{-4/3})$ anytime lower bound of Tsai et al. (2026), respectively. Both results continue to hold when the stepsizes may be negative. Our anytime lower bound also shows that the $O(n^{-\log_2(1+\sqrt{2})})$ rate of non-anytime silver schedules (Altschuler and Parrilo, 2025; Grimmer et al., 2025) is unattainable in the anytime setting. This establishes a strict separation between the two settings.

==> figures/stepsize-chronology-body.tex <==
% Drawn inside a TikZ scope whose x- and y-scales are set by the caller.
\foreach \x/\h in {
  0/.55,1/1.18,3/.72,4/1.62,
  5/.62,6/.86,8/1.35,9/2.05,
  12/1.60,13/.55,14/1.30,16/.74,17/1.80,
  18/.55,20/.85}{
  \pgfmathsetmacro{\baseh}{min(\h,1)}
  \fill[baseblue] (\x-.18,0) rectangle (\x+.18,\baseh);
  \draw[baseblueedge!80!black,line width=.35pt]
    (\x-.18,0) rectangle (\x+.18,\baseh);
  \pgfmathtruncatemacro{\islong}{\h>1}
  \ifnum\islong=1
    \fill[tailgold!65] (\x-.18,1) rectangle (\x+.18,\h);
    \draw[tailgold!70!black,line width=.35pt]
      (\x-.18,1) rectangle (\x+.18,\h);
  \fi
}

\foreach \x/\h/\lab in {
  4/1.62/t_1,9/2.05/t_2,12/1.60/t_{q-1},17/1.80/t_q}{
  \fill[selectedpurple!82] (\x-.18,1) rectangle (\x+.18,\h);
  \draw[selectedpurple!70!black,line width=.4pt]
    (\x-.18,1) rectangle (\x+.18,\h);
  \node[above=2pt] at (\x,\h) {$\lab$};
}

\draw[densely dashed,softgray] (-.55,1)--(20.55,1);
\node[anchor=west,fill=white,inner xsep=2pt,inner ysep=1pt]
  at (20.25,1.10) {$h=1$};

\foreach \x in {2,7,10.5,15,19}
  \node at (\x,.25) {$\cdots$};

\node[below=2pt] at (0,0) {$h_1$};
\node[below=2pt] at (4,0) {$h_{t_1}$};
\node[below=2pt] at (9,0) {$h_{t_2}$};
\node[below=2pt] at (12,0) {$h_{t_{q-1}}$};
\node[below=2pt] at (17,0) {$h_{t_q}$};
\node[below=2pt] at (20,0) {$h_n$};

\draw[decorate,decoration={brace,mirror,amplitude=3.5pt}]
  (-.30,-.60)--(3.30,-.60) node[midway,below=5pt] {$S_1$};
\draw[decorate,decoration={brace,mirror,amplitude=3.5pt}]
  (4.70,-.60)--(8.30,-.60) node[midway,below=5pt] {$S_2$};
\node at (10.50,-.82) {$\cdots$};
\draw[decorate,decoration={brace,mirror,amplitude=3.5pt}]
  (12.70,-.60)--(16.30,-.60) node[midway,below=5pt] {$S_q$};
\draw[decorate,decoration={brace,mirror,amplitude=3.5pt}]
  (17.70,-.60)--(20.30,-.60) node[midway,below=5pt] {$S_{q+1}$};

